Symmetry, Geometry, Topology and Spin: Heisenberg spins in the continuum limit/magnetic vesicles

In this thesis I present my research on the exotic configurations of antiferromagnetic systems characterised by a topological invariant. The research presented outlines the construction of novel local antiferromagnetic degrees of freedom for low dimensional antiferromagnetic lattices. This new construction reproduces the real division algebra hierarchy satisfied by the nonlinear sigma-model and reveals the presence of a novel local gauge field. I have also studied elastic magnetic vesicles of spherical and toric genus in the presence of a magnetic soliton. My studies reveal a global shrinking, with local swellings in the regions where the soliton presents a spin-flip. The geometrical origin of this novel phenomena led me to interpret the geometric frustration of magnetic vesicles as the competition between the two topological orders present. The microscopic mechanism and topological competition suggested above go beyond the scope of this thesis, providing a microscopic explanation for the Fermi-Bose transmutation and a way to deal with this type of exotic physics.

==> babelbst.tex <==
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% localbabel.dtx  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from babelbst.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file localbabel.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\ProvidesFile{babelbst.tex}
  [1999/03/29 Local LaTeX configuration file]
\iflanguage{english}{\loadlocalcfg{englishbst}}{}
\iflanguage{french}{\loadlocalcfg{frenchbst}}{}
\endinput
%%
%% End of file `babelbst.tex'.


==> gtsAbstract-fr.tex <==
%% `gtsAbstract-fr.TeX' LaTeX input file | see the driver file `gtsAbstracts.TeX'!
%% last major modification: 1999/05/24
%%
\ProvidesFile{gtsAbstract-fr.tex}[1999/06/01 v0.9b GTS project: French Abstract]
Lors de cette thèse mes recherches
se sont principalement orientées vers l'étude
de systèmes antiferromagnétiques
en présence de configurations antiferromagnétiques
exotiques caractérisées par un invariant topologique.
\bigskip

De multiples tentatives infructueuses
pour mener à terme
le passage à une théorie des champs continue
du modèle antiferromagnétique de Heisenberg
sur le réseau triangulaire
dans la perspective de mettre en évidence
la présence du terme de Hopf dans le Lagrangien
m'ont conduits à esquisser
pour les réseaux antiferromagnétiques
de basse dimension
la construction de nouveaux
degrés de liberté antiferromagnétiques locaux.
Cette construction originale reproduit
la hiérarchie des algèbres réelles à divisions
vérifiée par le modèle $\sigma$ non-linéaire
(limite continue du Hamiltonien de Heisenberg classique
en dimension deux)
et révèle la présence d'un champs de jauge locale inédit.
Surtout
cette construction algébrique m'amène
à suggérer un nouveau processus microscopique
qui serait à l'origine du terme de Hopf,
d'états antiferromagnétiques topologiques
(caractérisés par l'indice de Pontrjagin)
et de la transmutation de Fermi-Bose
(supraconductivité).

\medskip
En outre
j'ai mis en évidence
pour des membranes magnétiques souples
de genre topologique sphérique et torique
en présence d'un soliton magnétique
l'existence d'un rétrécissement global
renflé localement aux vagues du soliton.
L'origine géométrique de ce phénomène inédit
m'a amené à interpréter
la frustration géométrique des membranes magnétiques souples
comme la compétition
entre les deux ordres topologiques présents
(décrits par l'indice de Pontrjagin du soliton
et le genre de la membrane).


\bigskip
Le processus microscopique
et la compétition topologique suggérés
élargissent le champs d'investigation initial
en fournissant une origine microscopique
à la transmutation de Fermi-Bose
et un moyen de traquer cette physique exotique.
\endinput
%%
%% End of file `gtsAbstract-fr.TeX'.


==> gtsAbstract-uk.tex <==
%% `gtsAbstract-uk.TeX' LaTeX input file | see the driver file `gtsAbstracts.TeX'!
%% last major modification: 1999/05/31
%%
\ProvidesFile{gtsAbstract-uk.tex}[1999/06/01 v0.9b GTS project: English Abstract]

In this thesis I present my research on
the exotic configurations of
antiferromagnetic
systems characterised by a topological invariant.
\bigskip

It is expected that taking the continuum limit of the
antiferromagnetic Heisenberg model on the triangular lattice gives
rise to a Lagrangian with a Hopf term.
The research presented in this thesis shows that the continuum
limit is much more difficult to achieve than may be expected.
This difficulty
led me to outline  the construction of novel local antiferromagnetic degrees of
freedom for low dimensional antiferromagnetic
lattices.
This new construction reproduces the real division
algebra hierarchy satisfied by the nonlinear $\sigma$-model
(which corresponds to the continuum limit of the Heisenberg Hamiltonian
for classical isotropic antiferromagnets
in two dimensions)
and reveals the presence of a novel local gauge field.
This algebraic construction
leads me to suggest a new microscopic
mechanism which should give rise to the Hopf term,
as well as antiferromagnetic topological states
(characterised by the Pontrjagin index),
and the Fermi-Bose transmutation
(superconductivity).


\medskip
In this thesis I have also studied
elastic magnetic vesicles
of spherical and toric genus in the presence of
a magnetic soliton.
My studies reveal a global shrinking,
with local swellings
in the regions where the soliton presents a spin-flip.
The geometrical origin of this novel phenomena
led me to interpret
the geometric frustration of magnetic vesicles
as the competition between
the two topological orders present
(one described by the Pontrjagin index of the soliton
and the other by the genus of the vesicle).

\bigskip
The microscopic mechanism
and topological competition suggested
above go beyond the scope of this thesis,
providing a microscopic explanation
for the Fermi-Bose transmutation
and a way to deal with this type of exotic physics.
\endinput
%%
%% End of file `gtsAbstract-uk.TeX'.


==> gtsAbstracts.tex <==
%% `gtsAbstracts.TeX' LaTeX input file | see the driver file `gtsThesis.TeX'!
%% last major modification: 1999/05/24
%%
\ProvidesFile{gtsAbstracts.tex}[1999/05/23 v0.7b GTS project: Abstracts]
\begin{otherlanguage}{french}
\specialchapteropenleft{\abstractname}
\begin{introduction}
\input{gtsAbstract-fr}
\end{introduction}
\end{otherlanguage}

\begin{otherlanguage}{english}
\specialchapter{\abstractname}
\begin{introduction}
\input{gtsAbstract-uk}
\end{introduction}
\end{otherlanguage}
\endinput
%%
%% End of file `gtsAbstracts.TeX'.


==> gtsPreamble.tex <==
%% `gtsPreamble.TeX' LaTeX input file | see the driver file `gtsThesis.TeX'!
%% last major modification: 1999/05/19
%%
\ProvidesFile{gtsPreamble.tex}[1999/06/05 v0.95b GTS project: Preamble]
\specialchapter{Remerciements}
\label{chp/preamble}
Ce travail a été effectué
à l'\textsc{Université de Cergy-Pontoise}
au sein du \textsc{Laboratoire de Physique Théorique et Modélisation}
dirigé par \textsc{Hung~The~DIEP}.

\bigskip
Je souhaite avant tout remercier
\textsc{Rossen~DANDOLOFF}
de m'avoir proposé ce sujet de thèse,
de m'avoir dirigé et aidé dans mes travaux,
et de m'avoir témoigné toute sa confiance.
Ses conseils, ses suggestions,
ses encouragements et son aide
m'ont été très utiles pour mener
ce travail à son terme.
\bigskip

Je remercie
\textsc{Karol~PENSON} et \textsc{Avadh~SAXENA}
d'avoir accepté d'être {\thesisreportername}
de mes recherches.
J'exprime également toute ma gratitude
envers les autres membres du Jury :
\textsc{Jean-François~SADOC},
{\Madamabbrname} \textsc{Radha~BALAKRISHNAN},
\textsc{Jérôme~LEON} et
\textsc{Tuong~TRUONG}.

\bigskip
Je suis redevable à \textsc{Hung~The~DIEP}
d'avoir permis le bon déroulement
de mon séjour au \textsc{LPTM}.
Mes remerciements vont aussi
à tous les membres du laboratoire
avec qui j'ai eu de fructueuses discussions.

\endinput
%%
%% End of file `gtsPreamble.TeX'.

